Credit Attribution and Stable Compression

Credit attribution is crucial across various fields. In academic research, proper citation acknowledges prior work and establishes original contributions. Similarly, in generative models, such as those trained on existing artworks or music, it is important to ensure that any generated content influenced by these works appropriately credits the original creators. We study credit attribution by machine learning algorithms. We propose new definitions--relaxations of Differential Privacy--that weaken the stability guarantees for a designated subset of $k$ datapoints. These $k$ datapoints can be used non-stably with permission from their owners, potentially in exchange for compensation. Meanwhile, the remaining datapoints are guaranteed to have no significant influence on the algorithm's output. Our framework extends well-studied notions of stability, including Differential Privacy ($k = 0$), differentially private learning with public data (where the $k$ public datapoints are fixed in advance), and stable sample compression (where the $k$ datapoints are selected adaptively by the algorithm). We examine the expressive power of these stability notions within the PAC learning framework, provide a comprehensive characterization of learnability for algorithms adhering to these principles, and propose directions and questions for future research.

==> intro0.tex <==

\section{Introduction}

In many tasks that use Machine Learning algorithms one is also required to give proper \emph{credit attribution}. For example, consider a model that is trained on scientific papers and is required to reason about facts and figures based on existing literature. Most academic literature is protected under copyright licence such as CC-BY 4.0 that allows to distribute, remix, adapt, and build upon the material in any medium or format, so long as attribution is given to the creator. In another setting, a learner that needs to output generative content, such as images or music, might wish to allow generating \emph{derivative works} even of copyrighted materials, but without violating the creator's right (either by proper attribution or by monetary compensation based on context and licensing).

The increasing use of ML algorithms, and need of greater transparency, is also highlighted by regulations such as the recently implemented EU AI Act, which mandates the disclosure of training data \cite{IViR2023}. However, disclosure of training data and proper attribution are not necessarily equivalent. In particular, mere transparency of the dataset does not disclose whether certain elements of certain content have been derived, nor does it provide proper attribution where a certain content is heavily built upon. For that reason, there is a need to develop more nuanced mathematical notions and definitions that will enable learning under the constraint that works are properly attributed. This paper focuses on this challenge, and we explore theoretical models of \emph{credit attribution} with an attempt to provide rigorous and meaningful definitions to the task.

Credit attribution is a part of a much greater problem of learning under \emph{copyright} constraints. The rise of copyright issues in machine learning models is becoming increasingly prominent as these models are trained on vast amounts of data, some of which can be copyrighted. Consequently, the resulting models might implicitly contain copies of copyrighted data from their training sets. 
Previous work suggests it may be mathematically challenging to capture algorithms that protect copyrights like Differential Privacy does for privacy protection. In more detail, attempts to regulate copyright often focus on protection against \emph{substantial similarity} between output content and training data, for example by employing stable algorithms that are not sensitive to individual training points \cite{bousquet2020synthetic, vyas2023provable, scheffler2022formalizing}. This is an important aspect of copyright, however, substantial similarity is only a piece of the puzzle. In reality copyright law can even encourage using original elements of copyrighted works, in certain circumstances, such as \emph{de minimis
quotations}, transformative use, and other types of \emph{fair uses} such as learning and research \cite{elkin2023can}. To fully utilize ML in many practical scenarios, it is also desirable that learning models will be allowed to use original elements in a similar manner. 

A starting point, for dealing with this second piece of the puzzle, is the design of algorithms that, on the one hand are allowed to use copyrighted material and even be, heavily, influenced by it. But, to mitigate, we require that the algorithm provides proper attribution. Such models can allow, in turn, for the user to inspect such influences and verify that they conform with the standard of the law, or perform necessary measures (such as monetary compensation, request for permission etc.). Despite credit attribution being narrower in scope than copyrights in general, even this concept may be nuanced to be captured mathematically akin to Differential Privacy. Therefore, we focus on formalizing a specific (but arguably basic) aspect of it --- \emph{impartial attribution}: 
\begin{quote}
This principle asserts that any previous work that influenced the result should be credited.
In other words, if the creator of a work \(W\) does not acknowledge another work \(W'\), they could still produce \(W\) without any knowledge of~\(W'\). 
\end{quote}
For example, an argument based on this principle in the extreme case when \(W=W'\) is found in a U.S. Supreme Court opinion: 
\begin{quote}
\emph{“\ldots a work may be original even though it closely resembles other works, so long as the similarity is fortuitous, not the result of copying. To illustrate, assume that two poets, each ignorant of the other, compose identical poems. Neither work is novel, yet both are original\ldots”}
\end{quote}
\begin{flushright}
\textit{--- Feist Publications, Inc.\ v.\ Rural Telephone Service Company, Inc.\ 499 U.S.\ 340 (1991)}
\end{flushright}
